On the convergence of dynamic implementations of Hamiltonian Monte Carlo and No U-Turn Samplers

There is substantial empirical evidence about the success of dynamic implementations of Hamiltonian Monte Carlo (HMC), such as the No U-Turn Sampler (NUTS), in many challenging inference problems but theoretical results about their behavior are scarce. The aim of this paper is to fill this gap. More precisely, we consider a general class of MCMC algorithms we call dynamic HMC. We show that this general framework encompasses NUTS as a particular case, implying the invariance of the target distribution as a by-product. Second, we establish conditions under which NUTS is irreducible and aperiodic and as a corrolary ergodic. Under conditions similar to the ones existing for HMC, we also show that NUTS is geometrically ergodic. Finally, we improve existing convergence results for HMC showing that this method is ergodic without any boundedness condition on the stepsize and the number of leapfrog steps, in the case where the target is a perturbation of a Gaussian distribution.

==> proof/ergodicity_NUTS.tex <==



The proof of \Cref{thm:ergodicity_compile} is split into the proofs of the previous statements.
The presented proof can be extended to different choices of stopping time and index selection kernel $\rmqq_h$, 
but it is out of the paper's scope and relegated to future work.
First we show a prelimenary Lemma used to prove that the stopping time is locally constant in \Cref{lemma:nuts-locally-constant-trajectories}.
We introduce the sets
\begin{equation}
\label{eq:top_scru}
\scrU^{(K)}(a)=\{(q_0,p_0) \in (\mathbb{R}^d)^2\,:\, a\in \scrU^{(K)}(q_0,p_0) \} 
\end{equation} 
for any $K\in [\Kmax]$ and $a\in B_K$ where $\scrU^{(K)}(q_0,p_0)$ for $q_0,p_0\in (\Rset^d)^2$ is defined in \eqref{eq:scrU}. 
\begin{lemma}
\label{lemma:scru_open}
Under \Cref{hyp:regularity},
for any $K,K'\in [\Kmax]$, $a\in B_K$ and $q_0,p_0 \in \Rset^d$, 
$\scrU^{(K)}(a)$ (defined in \eqref{eq:top_scru}) is open and
$\scrU^{(K')}(a|_{K'})\subset \scrU^{(K)}(a)$ when $K>K'$.
Moreover, under \Cref{hyp:3}$(h,\Kmax)$, for any $q\in \Rset^d$, the following set is dense, 
\begin{equation}
   \label{eq:scrU-0}
   \msu_{q,-0}=\{ p\in \Rset^d: q,p\notin \partial \scrU^{(K)}(a),\, K\in [\Kmax],\, a\in B_K \} \eqsp .
\end{equation}
\end{lemma}
\begin{proof}[Proof of \Cref{lemma:scru_open}]
\input{proof/ergodicity_NUTS/lemma_scruopen.tex}
\end{proof}

In the following, we will often work with a fixed binary sequence $a = (a_k)_{k=0}^{\Kmax-1}\in B_{\Kmax}$, to this end, for all $q, p \in \mathbb{R}^d$ we set
\begin{equation}
S_a(q, p) = S(a,q,p),\ee  K_{f,a}(q,p)=(S_a(q, p)-1) \wedge \Kmax
\end{equation}
so that the index set constructed by the NUTS algorithm 
starting at $(q, p) \in (\Rset^d)^2$ is $B_{K_{f,a}(q,p)}(a|_{K_{f,a}(q,p)})$ when the Bernoulli variables $(V_k)_{k=0}^{\Kmax-1}$ take the values $a=(a_k)_{k=0}^{\Kmax-1}$.

\begin{lemma}
\label{lemma:nuts-locally-constant-trajectories}
% Let $a \in B_{\Kmax}$ and
% $$\mathrm{G}_a=\{ (q_0,p_0)\in (\mathbb{R}^d)^2,\ee r',r'' > 0, K \in [\Kmax]: $$
% $$K_{f,a}(q,p) = K, \ee(q, p) \in \mathrm{B}(q_0, r') \times \mathrm{B}(p_0, r'')\}$$
% $\mathrm{G}$ is a dense open set such that for any $q,p\in \mathrm{Y}$ and any $\epsilon>0$ there exists $p_\epsilon\in \mathrm{B}(p,\epsilon)$ such that $q,p_\epsilon\in G$.
% Moreover, if $q,p\notin \in \mathrm{G}_a $ then there exists $K\in [\Kmax]$ such that $q,p\in \partial \scrU^{(K)}(a|_K)$.

% Let $a \in B_{K_{\mathrm{max}}}$.
% There exists a dense open set $G' \subset (\Rset^d)^2$ such that for every $(q_0, p_0) \in G'$ there exist an $r' > 0$, $r'' > 0$ and $K \in \mathbb{N}$ such that $(S_a(q, p)-1) \wedge K_{\mathrm{max}} = K$ for all $(q, p) \in \mathrm{B}(q_0, r') \times \mathrm{B}(p_0, r'')$.

For all $a \in B_{\Kmax}$ there exists a dense open set $\mathrm{G}_a \subset (\mathbb{R}^d)^2$ such that $(q, p) \mapsto K_{f, a}(q, p)$ is locally constant on $\mathrm{G}_a$, i.e. for any $(q_0, p_0) \in \mathrm{G}_a$ there exists an open neighborhood $U \subset \mathrm{G}_a$ containing $(q_0, p_0)$ such that $K_{f, a}$ is constant on $U$.

% Moreover, recalling the set $\mathrm{Y} \subset (\mathbb{R}^2)$ from \eqref{eq:set-Y} and \eqref{eq:set-Delta}, under the hypotheses of Proposition \ref{prop:condition_check} for any $(q, p) \in \mathrm{Y}$ and $\epsilon > 0$ there exists a $p_\epsilon \in \mathrm{B}(p, \epsilon)$ such that $(q, p_\epsilon) \in \mathrm{G}_a$.
Moreover, under the hypotheses of Proposition \ref{prop:condition_check}, for any $(q, p) \in (\Rset^d)^2$ and $\epsilon > 0$ small enough there exists a $p_\epsilon \in \mathrm{B}(p, \epsilon)$ such that $(q, p_\epsilon) \in \mathrm{G}_a$.
\end{lemma}

\begin{proof}
\input{proof/ergodicity_NUTS/lemma_G_a.tex}
\end{proof}

\begin{remark}
In slightly less precise terms, this lemma says that the integer-valued function $(q,p) \in (\Rset^d)^2\mapsto S_a(q,p)$ is continuous in $\mathrm{G}_a$ and that nearly every point is in $\mathrm{G}_a$ if we allow a little perturbation of the initial momentum $p$.
\end{remark}

\begin{proof}[Proof of \Cref{prop:condition_check}]
\input{proof/ergodicity_NUTS/prop_small_stepsize.tex}
\end{proof}



% \begin{remark}
% In the last proof, the condition on the stepsize $h>0$,
% $$[(1+h \ltt_1^{\frac{1}{2}}\mathcal{V}(h \ltt_1^\frac{1}{2}))^{2^{\Kmax}}-1]<\frac{1}{4}$$
% is particularly restrictive.
% \end{remark}

\begin{proof}[Proof of \Cref{prop:condition_check_gaussian}]
\input{proof/ergodicity_NUTS/prop_gaussian.tex}
\end{proof}


\begin{proof}[Proof of \Cref{thm:1nuts-small-sets}.] 
\input{proof/ergodicity_NUTS/1small.tex}
\end{proof}

% \begin{remark}
% % TODO
% Comment for us.
% In the last proof, we use the condition on the step size $h>0$,
% $$\ltt_1 h^2 < 2 \big(1 - \cos \frac{\pi}{2^{\Kmax}}\big) $$
% Can we relax this condition, using the no uturn criteria ?

% \end{remark}

\begin{proof}[Proof of \Cref{thm:nuts-accessibility}.]
\input{proof/ergodicity_NUTS/accessibility.tex}
\end{proof}

% \begin{remark}
% In the last proof, we did not use any condition on the stepsize except to control stopping time.
% \end{remark}


%We denote by $q_T= \operatorname{proj}_1 \Phiverlet[h][T](q_0,p_0)$ for $T\in \nset^*$. In the proofs, we will use several times the argument that if a property on $q_T$ is true provided that $p_0 \in \mathrm{B}(0,r)$  with $r>0$ then the property is true for $q_{-T}$ since 
%\begin{equation}
%   \label{eq:symmetry_remark}
%  \operatorname{proj}_1 \Phiverlet[h][-T](q_0,p_0)=\operatorname{proj}_1 \Phiverlet[h][T](q_0,-p_0) 
%\end{equation}

% \begin{proof}[Proof of \Cref{prop:aperiodicity}]
%     we show that there exists $q_m\in \Rset^d$ and $r_0>0$ such that for any $r\in ]0,r_0[$ and for any $q\in \mathrm{B}(q_m,r)$:
%     $$\ee \KkerU_h(q,\mathrm{B}(q_m,r)) >0 $$
%     which is a sufficient condition to prove the aperiodicity since the chain is irreducible.
%     \miika{Details to be checked}

%     Let $q_0,p_0\in \Rset^d$ and denote by $q_i,p_i=\Phiverlet[h][i](q_0,p_0)$.
%      we show that when we sample $p_0$ in some ball $\mathrm{B}(q_0,r')\subset \Rset^d$, we reject the proposition of \Cref{alg:nuts-doubling} with positive probability
%      and we stay at $q_0$. 
%      If we detect a U turn between $q_0$ and $q_1$,
%       we stay in $q_0$ with positive probability when $\tpi(q_1,p_1)<\tpi(q_0,p_0)$.
%      We want to find a condition on $p_0$ such that $p_1^\top(q_1-q_0)<0$ to activate the U-turn condition and then to show that $\tpi(q_1,p_1)<\tpi(q_0,p_0)$.

%       If forall $q_0\in \Rset^d$ we have $\nabla U(q_0)=0$, $U$ is constant on $\Rset^d$ (because $U\in C^1(\Rset^d)$) which implies $\pi$ uniform on $\Rset^d$ which is not possible.
%      Therefore, it exists $q_0\in \Rset^d$ such that $\nabla U(q_0)\neq 0 $.
% \todo{SG: the proof should be mchanged, maybe we can use directly the accessibility}
%       We assume $ p_0=(h/2+\alpha)\nabla U(q_0)$ with $\alpha>0$ and $\nabla U(q_0)\neq 0 $. Then,
%      we have:
%      \begin{align}
%      &q_1=q_0+h\alpha \nabla U(q_0) \eqsp ,\\
%      &p_1=(\alpha-\frac{h}{2}) \nabla U(q_0)+\underbrace{\frac{h}{2}(-\nabla U(q_1)+\nabla U(q_0))}_{=\Delta(\alpha)}\eqsp , \\
%      & p_1^\top(q_1-q_0)= 
%         h\alpha (\alpha-\frac{h}{2}) |\nabla U(q_0)|^2+
%         h\alpha \nabla U(q_0)^\top\Delta(\alpha)\eqsp , 
%     \end{align}
%     With \Cref{hyp:3}-\ref{hyp:item_ii_homeo}, we have $|\Delta(\alpha)|\leq \alpha |\nabla U(q_0)|(h^2 \ltt_1)/2 $, then by assuming $\alpha \in ]0,\min(h/4,1/4)[$:
%     $$ p_1^\top(q_1-q_0)\leq h^2\alpha |\nabla U(q_0)|^2 [- \frac{1}{4}+\frac{h \ltt_1 }{2}\alpha ]\eqsp ,$$
%     $$- \frac{1}{4}+\frac{h \ltt_1 }{2}\alpha \leq - \frac{1}{4}+\frac{h^2 \ltt_1 }{2} \times \frac{1}{4} <0\eqsp , $$
%     since $(h^2 \ltt_1)/2<1$, which gives $p_1^\top(q_1-q_0)<0$.
%      There is a U-turn when $p_0=(h/2+\alpha)\nabla U(q_0)$ with $\alpha \in ]0,\min(h/4,1/4)[ $, by continuity of $ p_0\in \Rset^d \to p_1^\top(q_1-q_0)$, this is true for $p_0$ belonging to a ball $B_1^\alpha$ centred on $(h+\alpha)\nabla U(q_0)$.

%      Now we want to show that $\tpi(q_1,p_1)<\tpi(q_0,p_0)$ for $p_0\in B_2^\alpha$ with $B_2^\alpha\subset B_1^\alpha$. This is true if 
%      $$|p_1|^2>|p_0|^2\ee \text{and} \ee U(q_1)>U(q_0) \eqsp .$$
%      To show the previous conditions, 
%      we prove it for $p_0=(h/2+\alpha)\nabla U(q_0)$ with $\alpha \in ]0,\min(h/4,1/4)[ $ then we conclude by using the continuity of the function
%      $p_0\in \Rset^d \to (|p_1|^2- |p_0|^2)/2+U(q_1)-U(q_0)$. We have,
%     $$ |p_1|^2-|p_0|^2=|\nabla U(q_0)|^2 [(\alpha-\frac{h}{2})^2-(\alpha+\frac{h}{2})^2]+2(\alpha -\frac{h}{2})\nabla U(q_0)^\top\Delta(\alpha)+|\Delta(\alpha)|^2 $$
%     $$ \leq \alpha h |\nabla U(q_0)|^2[-2 +\frac{h^2 \ltt_1 }{2}+\frac{h^3 \ltt_1^2 }{4}\alpha]<0 \eqsp . $$
%     by using that the gradient of $U$ is lypschitz,
%     $$ U(q_1)-U(q_0)\geq \nabla U(q_0)^\top (q_1-q_0)-\frac{\ltt_1}{2}|q_1-q_0|^2$$
%     $$ U(q_1)-U(q_0)\geq\alpha h |\nabla U(q_0)|^2[ 1- \frac{\ltt_1 h}{2} \alpha  ]>0 \eqsp .$$
%     We have proved that for any $ q_0 \in \Rset^d: \nabla U(q_0)\neq 0,\ee \KkerU_h(q_0,\{q_0\})>0$ since the interior of $B_2^\alpha$ is not empty. 
%     By continuity of $\nabla U$, it exists $q_m\in \Rset^d$ and $r_0>0$ such that for any $r\in ]0,r_0[$ and for any $q\in \mathrm{B}(q_m,r)$:
%     $$\ee \KkerU_h(q,\mathrm{B}(q_m,r)) >0 $$
% \end{proof}
% \begin{remark}
%     In the last proof we use the condition of stability.
% \end{remark}

\begin{proof}[Proof of the \Cref{thm:3small}]
%it lack only the case j=1 for the open set (to do at the end of demo on accessiblity)
\input{proof/ergodicity_NUTS/3small.tex}
\end{proof}

% \begin{remark}
% In the last proof, we did not use any condition on the stepsize.
% \end{remark}





\begin{proof}[Proof of \Cref{prop:condition_check_analytic}.]
\input{proof/ergodicity_NUTS/prop_real_analytic.tex}
\end{proof}


% \begin{remark}
% Considering $p_0 \mapsto \det \left( \frac{\partial q_T}{\partial p_0} \right)$ instead of $p_0 \mapsto p_0^\top (q_T - q_0)$, a similar argument is possible for showing that the $\psi_q$ in \Cref{hyp:3}-\ref{hyp:item_ii_homeo} is a local homeomorphism for almost all $q, p \in \Rset^d$.
% Namely, the image of $\mathcal{N}(0, M)$ under $\psi_q$ has mass $1$ and the image measure may be computed with the change of variables formula, showing that the determinant is nonzero in a set of positive measure.
% \end{remark}





% \begin{lemma}
%     \label{lemma:perturbation_df}
%     Assume \Cref{hyp:0gaussian_perturbation} and let $q_0\in \Rset^d$.
%     For any $T\in \Zset$,
%     there exists a constant $C(T,h,\Sigma,A_5,q_0)>0$ %depending only on $T,\, h,\, \Sigma,\,A_5$ and $q_0$
%      such that for any $p_0\in\Rset^d$,
%     \begin{equation}
%         \label{eq:dd_torecur_qtilde}
%         |\dd_{p_0}\tilde{q}_T(q_0,p_0)-\dd_{p_0} q_T(q_0,p_0)|\leq C(T,h,\Sigma,A_5) (|p_0|+1)^{\rho-2}\eqsp ,
%     \end{equation}

%     \begin{equation}
%         \label{eq:dd_torecur_ptilde}
%         |\dd_{p_0}\tilde{p}_T(q_0,p_0)-\dd_{p_0}p_T(q_0,p_0)|\leq C(T,h,\Sigma,A_5) (|p_0|+1)^{\rho-2}\eqsp .
%     \end{equation}
% \end{lemma}
% \begin{proof}
%     The result will be proved by a strong recurrence on $\Nset$ and extended to $\Zset$ by symmetry properties of $\Phiverlet[\cdot][(\cdot)] $.
%     As a prelimenary remark, observe that for any $i\in\Zset^* $ there exist $c(T,q_0,\Sigma,h),\,\tilde{c}(T,q_0,\Sigma,h)>0$ such that for any $p_0\in \Rset^d$,
%     \begin{equation}
%         \label{eq:pre_remark_df}
%         |q_i|\geq \tilde{c} |p_0|, \quad|\nabla^2 \tilde{U}(q_i)|\leq A_5(|q_i|+1)^{\rho-2} \leq c (|p_0|+1)^{\rho-2}\eqsp ,
%     \end{equation}
%      by using \Cref{lemma:gaussian_case} and \Cref{hyp:0gaussian_perturbation}.
%     For any $T\in \Nset$, \eqref{eq:dd_torecur_qtilde} is the hypothesis of reccurence $H(T)$.
%     $H(0)$ is straightforward since $\dd_{p_0}\tilde{q}_T=\dd_{p_0}q_T=0$  and $H(1)$ as well since for any $q_0,p_0\in (\Rset^d)^2$, $\dd_{p_0}\tilde{q}_1(q_0,p_0)=h \Idd=\dd_{p_0}q_1(q_0,p_0)$.
%     Let $T\in \Nset^*\setminus\{1\}$ such that $H(1),\ldots,H(T-1)$ and prove $H(T)$. For any $q_0,p_0\in (\Rset^d)^2$,
%     \begin{equation}
%         |\dd_{p_0}\tilde{q}_T(q_0,p_0)-\dd_{p_0} q_T(q_0,p_0)|\leq \sum_{i=1}^{T-1}(T-i)|\nabla^2 U(\tilde{q}_i)\dd_p \tilde{q}_i-\nabla^2 U_\Sigma(q_i)\dd_p q_i|\eqsp ,
%     \end{equation}
%     for any $i\in [T-1]$, noticing that $\nabla^2 U_\Sigma=\Sigma$,
%     \begin{equation}
%         |\nabla^2 U(\tilde{q}_i)\dd_p \tilde{q}_i-\nabla^2 U_\Sigma(q_i)\dd_p q_i|\leq |\Sigma(\dd_p q_i-\dd_p \tilde{q}_i)|+|\nabla^2 \tilde{U}(\tilde{q}_i)\dd_p \tilde{q}_i|\eqsp ,
%     \end{equation}
%     Combining the two previous inequalities with \eqref{eq:pre_remark_point} and the fact that $\dd_p \tilde{q}_i$ is bounded with \cite[Lemma 17]{Durmus2017-tf} (the bound depending on $h,T,A_5$ and $\Sigma$) and applying $H(i)$ for $i\in [T-1]$, it yields 
%     $H(T)$. For any $T\in \Nset$, $H(T)$ holds and the result extends to $T\in \Zset$ by using \eqref{eq:symmetry_remark}.
%     As in the proof of \Cref{lemma:perturbation_point}, we use \eqref{eq:dd_torecur_qtilde} to prove \eqref{eq:dd_torecur_ptilde} for any $T\in \Nset$ and we conclude by using symmetry properties of $\Phiverlet[\cdot][\cdot] $. 
% \end{proof}
% Ecrire sur la théorie du degré ?
% For any $t\in [0,1]$, we define 
% \begin{equation}
%     U_t=(1-t) U_\Sigma+tU=U_\Sigma +t \tilde{U}  
% \end{equation}
%  and its related leapfrog trajectories for any $T\in \Zset$ and $q_0,p_0\in (\Rset^d)^2$,
% \begin{equation}
%     q_T^t=\operatorname{proj}_1\Phiverlet[h][T](q_0,p_0),\quad p_{T}^t=\operatorname{proj}_2\Phiverlet[h][T](q_0,p_0)\eqsp .
% \end{equation} 
% We introduce for any $T_1,T_2,T\in\Zset^3$ with $T_1\neq T_2$ the functions employed to prove \Cref{hyp:3}.
% \begin{equation}
%     F_{q_0,t}^{(T_1,T_2)}:\,p_0\in \Rset^d\mapsto (p_{T_1}^t)^\top(q_{T_2}^t-q_{T_1}^t),\quad \psi_{q_0,t}^{(T)}:\,p_0\in \Rset^d \mapsto q_T^t\eqsp ,
% \end{equation}
% \begin{lemma}
%     \label{lemma:positive_quantities}
%     Assume \Cref{hyp:0gaussian_perturbation}. Then,
%     for any $q_0\in \Rset^d$ and $T_1,T_2,T\in \Zset^2\times \Zset^* $ with $T_1\neq T_2$, there exists a constant $c(T_1,T_2,T,q_0,h,\Sigma,A_5)>0$, such that for any $p_0\in \Rset^d$ with $|p_0|\geq c$, for any $t\in [0,1]$,
%     \begin{equation}
%         |\nabla F_{q_0,t}^{(T_1,T_2)}(p_0)|>0,\quad |F_{q_0,1}^{(T_1,T_2)}(p_0)|> 0, \quad \det(\dd \psi_{q_0,1}^{(T)}(p_0))\neq 0
%     \end{equation}
% \end{lemma}

% \begin{proof}
%     As a prelimenary remark, if $U$ satisfies \Cref{hyp:0gaussian_perturbation} then for any $t\in[0,1]$, $U_t$ satisfies \Cref{hyp:0gaussian_perturbation} with the same constant $A_5$, thus we can apply \Cref{lemma:perturbation_point}, \Cref{lemma:perturbation_df} independantly of $t\in[0,1]$.
%     Let $t\in [0,1]$, $q_0\in \Rset^d$ and $T_1,T_2,T\in \Zset^2 \in \Zset^*$ with $T_1\neq T_2$.
%     We prove the result for $\det(\dd \psi_{q_0,t}^{(T_1)}(p_0))$, then $\nabla F_{q_0,t}^{(T_1,T_2)}(p_0)$ and finally $F_{q_0,t}^{(T_1,T_2)}$ but their proof are nearly independant.
%     We have,
%     \begin{equation}
%         |\dd_{p_0} \psi_{q_0,1}^{(T)}-\dd_{p_0}\psi_{q_0,0}^{(T)} |=|\dd_{p_0} q_{T}^1- \dd_{p_0}q_{T}^0|\eqsp .
%     \end{equation}
%     By a straightforward application of \Cref{lemma:perturbation_df}, there exists a constant $C(T,h,\Sigma,A_5,q_0)>0$ such that for any $p_0\in\Rset^d$,
%     \begin{equation}
%         |\dd_{p_0} \psi_{q_0,1}^{(T)}(p_0)-\dd_{p_0}\psi_{q_0,0}^{(T)}(p_0) |\leq C(1+|p_0|)^{\varrho-2}\eqsp .
%     \end{equation}
%      Moreover, by \Cref{lemma:gaussian_case} there exists $G\in \mathrm{GL}(\Rset^d)$ such that for any $p_0\in \Rset^d$, $\dd_{p_0}\psi_{q_0,0}^{(T_1)}(p_0)=G$.
%       Then, it exists a function $f:p_0\in \Rset^d\mapsto f(p_0)\in \mathcal{M}_d$ such that $\dd_{p_0} \psi_{q_0,t}^{(T)}(p_0)=G(\Idd+f(p_0)) $ for any $p_0\in\Rset^d$ and $|f(p_0)|\to 0 $ as $|p_0|\to \infty$.
%        Since $\mathrm{GL}(\Rset^d)$ is open, we deduce that it exists $M_1(T,q_0,h,\Sigma,A_5)>0$ such that for any $p_0\in \Rset^d$ with $|p_0|\geq M_1$, we have $\det(\dd \psi_{q_0,1}^{(T)}(p_0))\neq 0$.

%      For any $p_0\in \Rset^d$,
%     \begin{equation}
%         \begin{multlined}
%             |F_{q_0,1}^{(T_1,T_2)}-F_{q_0,0}^{(T_1,T_2)}|\leq 
%         |(p_{T_1}^1-p_{T_1}^0)^\top(q_{T_2}^1-q_{T_1}^1)|\\+|(p_{T_1}^0)^\top[q_{T_2}^1-q_{T_1}^1-(q_{T_2}^0-q_{T_1}^0)]|
%     \end{multlined}
%     \end{equation}
%     Using \cite[Lemma 17]{Durmus2017-tf}, we notice that $p_0\in \Rset^d\mapsto |q_{T_2}^1-q_{T_1}^1|(q_0,p_0)$ and $p_0\in \Rset^d\mapsto |(p_{T_1}^0)|(q_0,p_0)$ are lipsichtz with a constant independant of $t$ and $q_0$, then using \Cref{lemma:perturbation_point},
%      there exists a constant $C(T_1,T_2,q_0,h,\Sigma,A_5)>0$ such that
%     \begin{equation}
%         |F_{q_0,1}^{(T_1,T_2)}(p_0)-F_{q_0,0}^{(T_1,T_2)}(p_0)|\leq C (1+|p_0|^{\rho}) \eqsp .
%     \end{equation}
%     We have that $p_0\in \Rset^d \mapsto F_{q_0,0}^{(T_1,T_2)}(p_0)$ is quadratic in $p_0$ since $h$ is chosen according to \Cref{lemma:gaussian_case} and thus there exist constants $c_1(T_1,T_2,\Sigma,h),\, c_2(T_1,T_2,h,q_0,\Sigma)>0$ such that for any $p_0\in\Rset^d$,
%     \begin{equation}
%         |F_{q_0,0}^{(T_1,T_2)}(p_0)|\geq c_1|p_0|^2-c_2(|p_0|+1)\eqsp .
%      \end{equation}
%      Then,
%     \begin{align}
%        |F_{q_0,1}^{(T_1,T_2)}(p_0)|&\geq |F_{q_0,0}^{(T_1,T_2)}(p_0)|- |F_{q_0,1}^{(T_1,T_2)}(p_0)-F_{q_0,0}^{(T_1,T_2)}(p_0)|\\
%         &\geq |p_0|^2(c_1-c_2\frac{(|p_0|+1)}{|p_0|^2}-C\frac{1+|p_0|^{\rho}}{|p_0|^2})-C\frac{1+|p_0|^{\rho}}{|p_0|^2})
%     \end{align}
%      Since $\rho<2$, we have that there exists a constant $M_2(T_1,T_2,q_0,h,\Sigma,A_5)>0 $ such that for any $p_0\in \Rset^d$ with $|p_0|\geq M_2 $, we have $|F_{q_0,1}^{(T_1,T_2)}(p_0)|>0$.

%      Then, write for any $p_0\in \Rset^d $
%      \begin{equation}
%         \nabla F_{q_0,t}^{(T_1,T_2)}(p_0)= (\dd_{p_0} p_{T_1}^t)^\top (q_{T_2}^t-q_{T_1}^t)+(\dd_{p_0} (q_{T_2}^t-q_{T_1}^t))^\top p_{T_1}^t\eqsp ,
%      \end{equation}

%      \begin{align}
%         &|\nabla F_{q_0,t}^{(T_1,T_2)}(p_0)-\nabla F_{q_0,0}^{(T_1,T_2)}(p_0)|\leq |(\dd_{p_0} p_{T_1}^t-\dd_{p_0} p_{T_1}^0)| |q_{T_2}^t-q_{T_1}^t|\\
%         &+|\dd_{p_0} (q_{T_2}^t-q_{T_1}^t)-\dd_{p_0} (q_{T_2}^0-q_{T_1}^0)| |p_{T_1}^t|\\
%         &+ |\dd_{p_0} p_{T_1}^0| |q_{T_2}^t-q_{T_1}^t-(q_{T_2}^0-q_{T_1}^0)|+|\dd_{p_0} (q_{T_2}^0-q_{T_1}^0)|| p_{T_1}^t-p_{T_1}^0|
%      \end{align}
%       applying \Cref{lemma:perturbation_point},\Cref{lemma:perturbation_df}, \cite[Lemma 17]{Durmus2017-tf} and noticing that $|\dd_{p_0} p_{T_1}^0|, |\dd_{p_0} (q_{T_2}^0-q_{T_1}^0)|$ are bounded by a constant $C'(h,T_1,T_2,\Sigma)>0$, there exists a constant $C(q_0,h,T_1,T_2,\Sigma,A_5)>0$ (independant of $t$) such that for any $p_0\in \Rset^d$,
%       \begin{equation}
%         |\nabla F_{q_0,t}^{(T_1,T_2)}(p_0)-\nabla F_{q_0,0}^{(T_1,T_2)}(p_0)|\leq C(1+|p_0|^{\rho-1})
%       \end{equation}
%     $\nabla F_{q_0,0}^{(T_1,T_2)}(\cdot)$ is linear not constant by \Cref{lemma:gaussian_case}, thus it exist constants 
%     \begin{equation}
%         c_1(h,T_1,T_2,\Sigma),c_2(h,T_1,T_2,\Sigma,q_0)>0
%     \end{equation}
%     such that for any $p_0\in\Rset^d$,
%      \begin{equation}
%         |\nabla F_{q_0,0}^{(T_1,T_2)}(p_0)|>c_1|p_0|-c_2
%      \end{equation}
%     Then, by applying a triangular inequality, for any $p_0\in \Rset^d$,
%     \begin{equation}
%         |\nabla F_{q_0,t}^{(T_1,T_2)}(p_0)|\geq c_1|p_0|-c_2-C(1+|p_0|^{\rho-1})\eqsp . 
%     \end{equation}
%     Therefore, it exists a constant $M_3(T_1,T_2,q_0,h,\Sigma,A_5)>0$ such that for any $p_0\in \Rset^d$ with $|p_0|\geq M_3$, we have $|\nabla F_{q_0,t}^{(T_1,T_2)}(p_0)|>0$.
%     Finally, we set $c$ as the maximum of $M_1,M_2,M_3$.
% \end{proof}

% \begin{proof}[Proof of \Cref{prop:gaussian_perturbated}]
%     Let $q_0\in \Rset^d$ and prove \Cref{hyp:3}-\ref{hyp:item_ii_homeo}.
%     We apply \Cref{lemma:positive_quantities} for any $T_1,T_2,T\in [-2^{\Kmax}+1:2^{\Kmax}-1]^3$ with $T_1\neq T_2$ and $T\neq 0$, it yields constants 
%     \begin{equation}
%         (c(T_1,T_2,T,q_0,h,\Sigma,A_5))_{T_1,T_2,T\in [-2^{\Kmax}+1:2^{\Kmax}-1]^3,\,T_2\neq T_1,\, T\neq 0}
%     \end{equation}
%     and we take their maximum $c_M(q_0,h,\Sigma,A_5)>0$.
%     Then, for any $t\in [0,1]$, $p_0\in \Rset^d$ with $|p_0|\geq c_M$ and $T_1,T_2,T \in[-2^{\Kmax}+1:2^{\Kmax}-1]^3$ with $T_1\neq T_2$ and $T\neq 0$ , 
%     \begin{equation}
%         \label{eq:cond_compile}
%         |\nabla F_{q_0,t}^{(T_1,T_2)}(p_0)|>0,\quad |F_{q_0,1}^{(T_1,T_2)}(p_0)|> 0, \quad \det(\dd \psi_{q_0,1}^{(T)}(p_0))\neq 0 \eqsp .
%     \end{equation}
%     We deduce that for any $p_0\in \Rset^d$ with $|p_0|\geq c_M$, $q_0,p_0 \notin \partial \scrU(a) $ for any $K\in[\Kmax]$ and any $a\in B_K$, morever for any $T\in [-2^{\Kmax}+1:2^{\Kmax}-1]\setminus \{0\}$
%     $\psi_{q_0,1}^{(T)}(p_0)$ is a $\mathrm{C}^1$-diffeomorphism by the local inversion theorem. Therefore, \Cref{hyp:3}-\ref{hyp:item_ii_homeo}.

%     Let $T_1,T_2\in [-2^{\Kmax}+1:2^{\Kmax}-1]^2$ with $T_1\neq T_2$ and $r> c_M$.
%     We set $\msd_r=\bar{\mathrm{B}}(0,r)$ and consider the homotopy $H: (t,p_0)\in [0,1]\times \msd_r\mapsto \nabla F_{q_0,t}^{(T_1,T_2)}(p_0) $.
%     We have that $0_d\in \Rset^d\setminus H([0,1]\times \partial \msd_r) $ by \eqref{eq:cond_compile} and by \cite[Proposition 2.4]{degreeouterelo2009mapping},
%     \begin{equation}
%         \operatorname{deg}(\nabla F_{q_0,1}^{(T_1,T_2)},\msd_r,0_d)=\operatorname{deg}(\nabla F_{q_0,0}^{(T_1,T_2)},\msd_r,0_d)\leq 1\eqsp. 
%     \end{equation}
%     $\operatorname{deg}(\nabla F_{q_0,0}^{(T_1,T_2)},\msd_r,0_d)\leq 1$ since $\nabla F_{q_0,0}^{(T_1,T_2)}$ is linear one-to-one map by \Cref{lemma:gaussian_case}.
%     $r$ can be chosen arbitrary large, thus $(\nabla F_{q_0,1}^{(T_1,T_2)})^{-1}(\{0\})$ is a singleton. Therefore, be setting 
%     \begin{equation}
%         \msy = \{q_0,p_0 \in (\Rset^d)^2:\, p_0 \notin \bigcup_{T_1,T_2\in [-2^{\Kmax}+1:2^{\Kmax}-1],\,T_1\neq T_2} (\nabla F_{q_0,1}^{(T_1,T_2)})^{-1}(\{0\}) \} \eqsp ,
%     \end{equation}
%     \Cref{hyp:3}-\ref{hyp:item_i_topo} follows with the same sketch of proof of \Cref{prop:condition_check} and the proof is complete.

% \end{proof}

% Now, the same result is true when $\Sigma \to 0$.
% \begin{assumption}
%     \label{hyp:0perturbation}
% There exists $\tilde{U}: \mathbb{R}^d \rightarrow \mathbb{R}$, twice continuously differentiable such that $U(q):=\tilde{U}(q)$ and there exist $A_5 \geq 0$ and $\varrho \in[1,2)$ such that for any $q, x \in \mathbb{R}^d$
% $$
% \begin{gathered}
% |\tilde{U}(q)| \leq A_5\left(1+|q|^{\varrho}\right), \quad|\nabla \tilde{U}(q)| \leq A_5\left(1+|q|^{\varrho-1}\right)\eqsp, \\
% |\nabla \tilde{U}(q)-\nabla \tilde{U}(x)| \leq A_5|q-x|,\quad |\nabla^2 \tilde{U}(q)|\leq A_5 (1+|q|)^{\varrho-2}\eqsp .
% \end{gathered}
% $$
% \end{assumption}
% \begin{proposition}
%     \label{prop:gaussian_perturbated_limit}
%     Assume \Cref{hyp:0perturbation}. There exists a countable set $\msh_0\subset \Rset_{\geq0}$ such that for any $\msm_h>0$ and $h\in (\Rset_{>0}\setminus \msh_0)\cap [0,\msm_h] $, \Cref{hyp:3} is satisfied.
% \end{proposition}
% \begin{proof}
% The same lines of the proof of \Cref{prop:gaussian_perturbated} apply, provided that we use \Cref{lemma:positive_quantities2} instead of \Cref{lemma:positive_quantities}. \Cref{lemma:positive_quantities2} is proved in the following.
% For this purpose, we introduce some notations. 

% Let $a\in [0,1]$ and $\msm_h>0$. Applying \Cref{lemma:gaussian_case} with $\Sigma= a\Idd$
% , there exists $\msh_0^a$ such that the conclusions of \Cref{lemma:gaussian_case} hold and let $h\in (\Rset_{>0}\setminus \msh_0^a)\cap [0,\msm_h]$. 
% For any $t\in [0,1]$, we define $\check{U}_{t,a}=(1-t)\tilde{U}+tU_{ a \Idd} $ and its related leapfrog trajectories for any $T\in \Zset$ and $q_0,p_0\in (\Rset^d)^2$,
% \begin{equation}
%     q_T^t=\operatorname{proj}_1\Phiverlet[h][T](q_0,p_0),\quad p_{T}^t=\operatorname{proj}_2\Phiverlet[h][T](q_0,p_0),\quad \ltt_1^t=\|\check{U}_t\|_{lip}\eqsp .
% \end{equation} 
% We introduce for any $T_1,T_2,T\in\Zset^3$ with $T_1\neq T_2$ the functions employed to prove \Cref{hyp:3}.
% \begin{equation}
%     F_{q_0,t,a}^{(T_1,T_2)}:\,p_0\in \Rset^d\mapsto (p_{T_1}^t)^\top(q_{T_2}^t-q_{T_1}^t),\quad \psi_{q_0,t,a}^{(T)}:\,p_0\in \Rset^d \mapsto q_T^t\eqsp .
% \end{equation}
% We index the previous functions by $a$ since it will be chosen wisely in the following depending on $\msm_h,T_1,T_2,T$ to establish the following result.
% \begin{lemma}
%     \label{lemma:positive_quantities2}
%     Assume \Cref{hyp:0perturbation}. Then, there exists a countable set $\msh_0\subset \Rset_{\geq0}$ such that for any $M>0$ and $h\in (\Rset_{>0}\setminus \msh_0)\cap [0,M] $,
%     for any $q_0\in \Rset^d$ and $T_1,T_2,T\in \Zset^3$ with $T_1\neq T_2$ and $T\neq 0$ , there exist constants 
%     \begin{equation}
%         c(T_1,T_2,T,q_0,h,A_5),\,c_a(T_1,T_2,T,\msm_h,A_5) >0
%     \end{equation}
%      and such that for any $p_0\in \Rset^d$ with $|p_0|\geq c$, for any $t\in [0,1]$ and $a\in ]0,c_A[$,
%     \begin{equation}
%         |\nabla F_{q_0,t,a}^{(T_1,T_2)}(p_0)|>0,\quad |F_{q_0,0,a}^{(T_1,T_2)}(p_0)|> 0, \quad \det(\dd \psi_{q_0,0,a}^{(T)}(p_0))\neq 0
%     \end{equation}
% \end{lemma}
% \begin{proof}
%     As a prelimenary remark,
%     for any $i\in \Zset^*$ and $t\in[0,1]$, by using \Cref{hyp:0perturbation}, \cite[Lemma 17]{Durmus2017-tf}, for any $p_0\in \Rset^d $,
%     \begin{equation}
%         \label{eq:lip_qt}
%         |q_i^t|\leq (\ltt_1^t)^{-\frac{1}{2}}(1+h (\ltt_1^t)^{\frac{1}{2}}\mathcal{V}(h (\ltt_1^t)^\frac{1}{2}))^{|i|} |p_0|+|q_0|\eqsp,
%     \end{equation}
%     where $\ltt_1^t\leq ta+A_5\leq A_5+1$ for any $t\in[0,1]$ and we denote by for any $T\in \Zset^*$, 
%     \begin{equation}
%         \tilde{c}_{lip}=\max_{0\leq j \leq |T|} (A_5)^{-\frac{1}{2}}(1+\msm_h (A_5+1)^{\frac{1}{2}}\mathcal{V}(\msm_h (A_5+1)^\frac{1}{2}))^{j}
%     \end{equation}
%     and by \eqref{eq:q_develop_nice},
%     \begin{align}
%         \label{eq:qt_minor}
%         |q_T^t|&\geq Th |p_0|-T^2h^2\sum_{i=0}^{T-1} |\nabla U(q_i^t)|\geq Th |p_0|-T^2h^2\sum_{i=0}^{T-1} (t a |q_i^t|+A_5 (|q_i^t|+1)^{\rho-1})\\
%         &\geq Th |p_0|-a T^2h^2\tilde{c}_{lip}|p_0|-T^2h^2 (A_5+1)(|p_0|^{\varrho-1}+1+|q_0|)
%     \end{align}
%     thus $ |q_T^t|\to \infty $ as $|p_0|\to \infty$ and $a <1/(T \msm_h\tilde{c}_{lip}) $ and the growth does not depend on $t$. Assume $a <1/(T \msm_h\tilde{c}_{lip}) $ in the following, then there exists $c_2(h,T,A_5,q_0)>0$ such that for any $p_0\in \Rset^d$,
%     \begin{equation}
%         \label{eq:hessian_converge}
%        | \nabla^2 \check{U}_{t,a}(q_T^t)-t a \Idd|\leq (1-t)  |\nabla^2 \tilde{U}(q_T^t)|\leq (1-t) A_5 (1+|q_T^t|)^{\varrho-2} \leq c_2(1+|p_0|)^{\varrho-2}
%     \end{equation}
%     and thus $\nabla^2 \check{U}_t(q_T^t)\to t a \Idd  $ as $|p_0| \to \infty$.

%     Let $q_0\in \Rset^d$ and $T_1,T_2,T \in \Zset^3$ with $T_1\neq T_2$ and $T\neq 0$.
%     From \eqref{eq:df_qq}, in the case $t=0$, we deduce that there exist a constant $M_1(h,T,A_5,q_0)>0$ and $\tilde{B}:p_0\mapsto \tilde{B}(p_0)\in \mathcal{M}_d$ such that for any $p_0\in (\Rset^d)$ with $|p_0|>M_1 $
%     \begin{equation}
%         \dd \psi_{q_0,0,a}^{(T)}(p_0)=T h (\Idd+\tilde{B}(p_0)),\quad \tilde{B}(p_0)\leq \frac{1}{2}\eqsp ,
%     \end{equation}
% then $\dd \psi_{q_0,0,a}^{(T_1)}(p_0)\in \mathrm{GL}(\Rset^d)$ and thus $\det(\dd \psi_{q_0,0}^{(T)}(p_0))\neq 0$.
% From \eqref{eq:phiver_q_develop} and \eqref{eq:phiver_p_develop}, for any $p_0\in \Rset^d$,
% \begin{equation}
% |F_{q_0,0,a}^{(T_1,T_2)}(p_0)|\geq (T_2-T_1)h |p_0|^2 - T^2\max(h^2,h^3)(\sum_{i=0}^T |\nabla U(q_i^0)|)^2\eqsp ,
% \end{equation}
% by applying \Cref{hyp:0perturbation} and \cite[Lemma 17]{Durmus2017-tf}, there exists a constant $c_2(h,T_1,T_2,A_5,q_0)>0$ such that for any $p_0\in \Rset^d$,
% \begin{equation}
%     |F_{q_0,0,a}^{(T_1,T_2)}(p_0)|\geq (T_2-T_1)h |p_0|^2\geq (T_2-T_1)h |p_0|^2 -c_2 |p_0|^{2(\varrho-1)}\eqsp .
% \end{equation}
% Since $\rho<2$, we have that there exists a constant $M_2(T_1,T_2,q_0,h,A_5)>0 $ such that for any $p_0\in \Rset^d$ with $|p_0|\geq M_2 $, we have $|F_{q_0,0,a}^{(T_1,T_2)}(p_0)|>0$.

% To bound from above $|\nabla F_{q_0,t,a}^{(T_1,T_2)}(p_0)|$, the same arguments employed in the proof \Cref{prop:condition_check} apply:
%  we bound the matrices $A_t,B_t$ (defined in \eqref{eq:A_def},\eqref{eq:B_def} respectively) related to $\check{U}_t$ independantly of $t$ in order to use \Cref{lemma:perp}.
%  To this end, for any $i \in [T_1,T_2] $, we have from \eqref{eq:lip_qt}, for any $p_0\in\Rset^d$,
%  \begin{equation}
%     |\nabla^2 \check{U}_{t,a}(q_i^t) \dd_p q_i^t(q_0,p_0)|\leq |\nabla^2 \check{U}_{t,a}(q_i^t) |\tilde{c}_{lip}\eqsp,
%  \end{equation}

% using \eqref{eq:hessian_converge}, we deduce that there exisits a constant $M_3'(h,T_1,T_2,A_5,\msm_h)>0$ such that for any $p_0\in \Rset^d$ with $|p_0|\geq M_3'$ and for any $t\in[0,1]$, we have,
% \begin{equation}
%     |\nabla^2 \check{U}_{t,a}(q_i^t) \dd_p q_i^t(q_0,p_0)|\leq 2ta \tilde{c}_{lip}\leq 2a \tilde{c}_{lip}\eqsp.
%  \end{equation}
% Using the expressions of $A_t,\,B_t$ (\eqref{eq:A_def},\eqref{eq:B_def} respectively), there exists $c_a(T_1,T_2,T,\msm_h,A_5)\in ] 0, 1/(T \msm_h\tilde{c}_{lip})[$, such that if $a\in ]0,c_5[$, we have
% $\max(|A_t|,|B_t|)<1/4$.
% Moreover, by using \eqref{eq:lip_qt}, we deduce that for $p_0$ large enough (taking $M_3$ larger if necessary), we have $q_{T_2}^t \neq q_{T_1}^t$ for any $t\in [0,1]$.
%  Therefore \Cref{lemma:perp} applies and we conclude that $|\nabla F_{q_0,t,a}^{(T_1,T_2)}(p_0)|>0$ for any $t\in [0,1]$ and for any $p_0\in \Rset^d$ with $|p_0|\geq M_3$.
%  Finally, we set $c$ as the maximum of $M_1,M_2,M_3$.
% \end{proof}
% To conclude the proof as in \Cref{prop:gaussian_perturbated}, let $q_0\in \Rset^d$ and $\msm_h>0$
% We apply \Cref{lemma:positive_quantities2} for any $T_1,T_2,T\in [-2^{\Kmax}+1:2^{\Kmax}-1]^3$ with $T_1\neq T_2$ and $T\neq 0$, it yields constants 
%     \begin{equation}
%         (c(T_1,T_2,T,\msm_h,A_5),c_a(T_1,T_2,T,q_0,\msm_h,A_5))_{T_1,T_2,T}
%     \end{equation}
%     and we take their maximum $c_M(q_0,h,\Sigma,A_5)>0$ for $c$ and their minimum for $c_a$. Let $a \in ]0,c_a[$.
%     Then, for any $t\in [0,1]$, $p_0\in \Rset^d$ with $|p_0|\geq c_M$ and $T_1,T_2,T \in[-2^{\Kmax}+1:2^{\Kmax}-1]^3$ with $T_1\neq T_2$ and $T\neq 0$ , 
%     \begin{equation}
%         \label{eq:cond_compile}
%         |\nabla F_{q_0,t,a}^{(T_1,T_2)}(p_0)|>0,\quad |F_{q_0,1,a}^{(T_1,T_2)}(p_0)|> 0, \quad \det(\dd \psi_{q_0,1,a}^{(T)}(p_0))\neq 0 \eqsp .
%     \end{equation}
%     Then, the same lines of the proof of \Cref{prop:gaussian_perturbated} applies where we have $\nabla F_{q_0,t,a}^{(T_1,T_2)},F_{q_0,1,a}^{(T_1,T_2)},\psi_{q_0,1,a}^{(T)}$ instead of $\nabla F_{q_0,t}^{(T_1,T_2)},F_{q_0,0}^{(T_1,T_2)},\psi_{q_0,0}^{(T)}$.

% \end{proof} 


